Robust Driving Control for Autonomous Vehicles: An Intelligent General-sum Constrained Adversarial Reinforcement Learning Approach

Deep reinforcement learning (DRL) has demonstrated remarkable success in developing autonomous driving policies. However, its vulnerability to adversarial attacks remains a critical barrier to real-world deployment. Although existing robust methods have achieved success, they still suffer from three key issues: (i) these methods are trained against myopic adversarial attacks, limiting their abilities to respond to more strategic threats, (ii) they have trouble causing truly safety-critical events (e.g., collisions), but instead often result in minor consequences, and (iii) these methods can introduce learning instability and policy drift during training due to the lack of robust constraints. To address these issues, we propose Intelligent General-sum Constrained Adversarial Reinforcement Learning (IGCARL), a novel robust autonomous driving approach that consists of a strategic targeted adversary and a robust driving agent. The strategic targeted adversary is designed to leverage the temporal decision-making capabilities of DRL to execute strategically coordinated multi-step attacks. In addition, it explicitly focuses on inducing safety-critical events by adopting a general-sum objective. The robust driving agent learns by interacting with the adversary to develop a robust autonomous driving policy against adversarial attacks. To ensure stable learning in adversarial environments and to mitigate policy drift caused by attacks, the agent is optimized under a constrained formulation. Extensive experiments show that IGCARL improves the success rate by at least 27.9% over state-of-the-art methods, demonstrating superior robustness to adversarial attacks and enhancing the safety and reliability of DRL-based autonomous driving.

==> Texbackup/1-backup.tex <==
\section{Introduction}

\IEEEPARstart{T}{he} rapid development of autonomous driving (AD) technology is reshaping transportation systems, with the potential to substantially improve road safety, mitigate traffic congestion, and enhance mobility \cite{zhao2025survey, sun2025sparsedrive}.
As a prominent AI paradigm, deep reinforcement learning (DRL) has achieved remarkable success in complex sequential decision-making tasks in recent years \cite{zhang2025embodied, guo2025deepseek}.
Its powerful decision-making capability makes it a promising approach for the realization of AD \cite{zhaoSurveyRecentAdvancements2024a,al-sharmanSelfLearnedAutonomousDriving2023}.
In recent studies, DRL-based methods have demonstrated effectiveness across a variety of driving tasks, including highway driving \cite{zhang2024integration, wang2025highway}, on-ramp merging \cite{liuReinforcementLearningBasedMultiLane2024, liOnRampMergingHighway2023}, and intersection navigation \cite{hoelEnsembleQuantileNetworks2023, zhangPredictiveTrajectoryPlanning2023}.

Despite these achievements, the safety and robustness of DRL-based AD policies remain critical factors for their real-world deployment \cite{huang2024human, zhang2025}. AD is inherently safety-critical with virtually no margin for error. Even small deviations, such as a slight steering overcorrection, can lead to safety-critical events, such as collisions \cite{wang2025uncertainty, zhaoSurveyRecentAdvancements2024a}. Notably, even well-trained DRL policies often exhibit significant vulnerabilities to adversarial attacks \cite{ding2023seeing, standenAdversarialMachineLearning2025}. 
Such attacks operate by injecting carefully crafted adversarial perturbations into the agent’s sensory inputs, such as camera images, LiDAR point clouds, or radar signals, to mislead the driving policy of the agent \cite{fan2024less_is_more}. 
Such vulnerabilities represent a critical bottleneck for deploying DRL in AD, where robustness is not merely desirable but essential.

Adversarial training has emerged as a widely used defense paradigm for improving the robustness of DRL agents against adversarial perturbations \cite{li2025enhancing, zhou2024adversarial}. 
The key idea is to enhance robustness by training a agent in competition with an adversary deliberately crafted to exploit its vulnerabilities through adversarial perturbations. 
While this technique has shown notable success in strengthening AD policies, existing methods still face at least \textbf{three critical challenges}.
\begin{itemize}
\item \textbf{Oversimplified Zero-Sum Reward Design:} Existing works typically formulate adversarial training as a two-player zero-sum game, where the adversary minimizes the agent’s cumulative reward \cite{heRobustDecisionMaking2023, wang2025, guoRobustTrainingMultiagent2025}, as shown in Fig.\ref{fig:framework}(a). 
While this design is common in other domains, it is not suit for AD.
In this context, an adversary’s primary objective is to induce safety-critical events, whereas a driving agent’s reward function must also account for efficiency and comfort.
Consequently, a zero-sum design may bias the adversary toward generating perturbations that affect efficiency or comfort, rather than causing serious safety-critical events~\cite{bai2025rat}. 
Therefore, the challenge lies in designing an adversary with an objective directly coupled to safety-critical events, ensuring that the training process exposes the most critical vulnerabilities.

\item  \textbf{Myopic Adversary Design:} Many existing adversaries adopt a greedy strategy, focusing on immediate gains at each timestep \cite{heRobustLaneChange2023, wangExplainableDeepAdversarial2024a, heTrustworthyAutonomousDriving2024a}, as shown in Fig.\ref{fig:framework}(b). 
For instance, the adversary may generate perturbations that maximize the agent’s action deviation at each time step \cite{heRobustDecisionMaking2023}.
While these perturbations may succeed in specific critical states, this myopic behavior neglects the temporal dynamics intrinsic to driving.
In reality, the effects of an action, such as a slight acceleration change, often manifest with delays, creating opportunities for long-horizon attacks.
A carefully planned sequence of perturbations can compound over time, ultimately inducing severe safety-critical events.
Consequently, the challenge lies in ensuring that agents remain robust against adversaries capable of strategic, multi-step attacks, rather than only against myopic, stepwise-optimal perturbations.

\item \textbf{Unconstrained Training Instability:} Existing agents are generally trained under the standard Markov Decision Process (MDP) framework, in which they freely explore and optimize their policies in the presence of adversarial perturbations \cite{ma2018improved, zhangCATClosedloopAdversarial2023, caiAdversarialStressTest2024, guoRobustTrainingMultiagent2025}, as shown in Fig.\ref{fig:framework}(c). 
This design overlooks that unconstrained exploration in perturbed dynamics can not only bias the learned policy but also induce training instability. 
The agent may mistake perturbed states as clean states, leading to a failure to learn the safe action distribution in unperturbed environments. 
Moreover, the dynamic nature of adversarial perturbations can further destabilize training, making policy optimization more challenging.
Consequently, the challenge lies in improving robustness against adversarial perturbations while maintaining reliable performance in clean environments.
\end{itemize}

Therefore, we introduce Intelligent General-sum Constrained Adversarial Reinforcement Learning (IGCARL), a novel robust AD approach to address the aforementioned challenges, as shown in Fig.\ref{fig:framework}(d). 
IGCARL consists of two key components, a strategic targeted adversary designed to find critical vulnerabilities and a robust driving agent trained to withstand the adversary. First, departing from myopic adversaries, the adversary leverages the temporal decision-making and long-term planning capabilities of DRL to generate multi-step, strategically coordinated attack sequences. Furthermore, unlike traditional zero-sum formulations, this adversary operates under a general-sum objective, with its reward explicitly decoupled from the agent’s reward. This design allows the adversary to focus directly on inducing safety-critical events. To enhance driving robustness against such an advanced adversary, we train a robust driving agent in the adversary-perturbed environment using adversarial training. Unlike the paradigm of unconstrained optimization, the agent employs constrained policy optimization. Specifically, we impose two key constraints: a collision risk constraint to limit high-risk behaviors and a policy consistency constraint to enforce policy consistency. These constraints jointly ensure stable learning and mitigate policy drift caused by adversarial perturbations. 
To the best of our knowledge, this is the first work to improve the robustness of autonomous driving policies against a stronger type of threat: strategic adversarial attacks that coordinate multiple steps to trigger safety-critical failures.
Our approach has the following advantages:

\begin{itemize}
  \item \textbf{Strategic Attacks:} The DRL-based adversary can plan multi-step, strategically coordinated attack sequences, overcoming the limitations of myopic, single-step attacks.
  \item \textbf{Worst-case Oriented Attacks:} The adversary explicitly focuses on inducing safety-critical events, such as collisions, rather than merely reducing the agent’s performance.
  \item \textbf{Stable Learning:} The robust driving agent is trained using constrained optimization, ensuring stable learning even under changing dynamics caused by adversarial perturbations.
  \item \textbf{Mitigation of Policy Drift:} The policy consistency constraint can prevent the driving policy from overfitting to adversarial perturbations, ensuring reliable performance under both adversarial and clean conditions.
  \item \textbf{Stable in Clean Environments:} The collision risk constraint can ensure the stable performance of the agent even in clean environments.
\end{itemize}

The remainder of this paper proceeds as follows. Section II reviews related work, and Section III details our proposed approach, IGCARL. We then present and analyze experimental results in Section IV, and finally conclude in Section V.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth, trim=0 10 10 10, clip]{figures/fig1.pdf} 
    \caption{Overview of IGCARL and its role in addressing key challenges.}
    \label{fig:framework}
\end{figure}



